Deterministic 3SUM-Hardness

As one of the three main pillars of fine-grained complexity theory, the 3SUM problem explains the hardness of many diverse polynomial-time problems via fine-grained reductions. Many of these reductions are either directly based on or heavily inspired by P\u{a}tra\c{s}cu's framework involving additive hashing and are thus randomized. Some selected reductions were derandomized in previous work [Chan, He; SOSA'20], but the current techniques are limited and a major fraction of the reductions remains randomized. In this work we gather a toolkit aimed to derandomize reductions based on additive hashing. Using this toolkit, we manage to derandomize almost all known 3SUM-hardness reductions. As technical highlights we derandomize the hardness reductions to (offline) Set Disjointness, (offline) Set Intersection and Triangle Listing -- these questions were explicitly left open in previous work [Kopelowitz, Pettie, Porat; SODA'16]. The few exceptions to our work fall into a special category of recent reductions based on structure-versus-randomness dichotomies. We expect that our toolkit can be readily applied to derandomize future reductions as well. As a conceptual innovation, our work thereby promotes the theory of deterministic 3SUM-hardness. As our second contribution, we prove that there is a deterministic universe reduction for 3SUM. Specifically, using additive hashing it is a standard trick to assume that the numbers in 3SUM have size at most $n^3$. We prove that this assumption is similarly valid for deterministic algorithms.

==> sections/notes.tex <==
\section*{Notes}
\paragraph{Papers with 3SUM LBs}

\sout{Higher lower bounds from 3SUM}

How Hard is it to Find (Honest) Witnesses?

\sout{Monochromatic triangles, intermediate matrix products, and convolutions}
%\nick{3-SUM $<=>$ MonoConvolution. Need: Reduction from 3-SUM to $n^{2/3}$ instances of AN-3-SUM of size $n^{2/3}$ and universe $n^{4/3}$. In combination with the universe-efficient self-reduction for AN-3SUM, only needs that AN-3SUM is hard over quadratic universes. Should be doable; I'll write a lemma.}

\sout{The Dynamic k-Mismatch Problem (Clifford et al)}% \adam{Seems to depend on the universe size bound for All Ints 3SUM}

\sout{Hardness of Detecting Abelian and Additive Square Factors in Strings}
%\nick{Needs that convolution-3SUM is hard over quadratic universes. Can probably be done; I'll write a lemma.}

\sout{Removing Additive Structure in 3SUM-Based Reductions}

\sout{Stronger 3-sum lower bounds for approximate distance oracles}

UNBALANCED TRIANGLE DETECTION AND ENUMERATION HARDNESS FOR UNIONS OF CONJUNCTIVE QUERIES

The Complexity of Boolean Conjunctive Queries with Intersection Joins

On the Hardness of Set Disjointness and Set Intersection with Bounded Universe

\sout{Popular conjectures imply strong lower bounds for dynamic problems.}
% \nick{At first glance: No tight lower bounds.}

\sout{Geometric reductions: Gajentann–Overmars, Erickson SODA'95, Hernandez-Barrera '96, Barequet and Har-Peled 2001, Soss-Erickson-Overmars, Gomez-Ramaswami-Toussaint} %\adam{Erickson and Henrandez-Barrera papers do not actually includem 3sum-based LBs}

\sout{Consequences of faster alignment of sequences.}
% \nick{Deterministic given the deterministic self reduction. Proves that the Local Alignment problem is 3-SUM hard.}

\sout{All non-trivial variants of 3-LDT are equivalent}

\sout{Finding, minimizing, and counting weighted subgraph}

\sout{Subcubic equivalences between path, matrix and triangle problems}

\sout{Zahra Jafargholi and Emanuele Viola. 3sum, 3xor, triangle}

\sout{On hardness of jumbled indexing}

\sout{Mind the gap: Essentially optimal algorithms for online dictionary matching with one gap.}
%\nick{Only via Triangle Listing}

\sout{Matching triangles and basing hardness on an extremely popular conjecture}

\sout{Amir Abboud and Kevin Lewi. Exact weight subgraphs and the k-sum conjecture}

\sout{Mihai Patrascu and Ryan Williams. On the possibility of faster sat algorithms}

\sout{Ilya Baran, Erik D. Demaine, and Mihai Patrascu. Subquadratic algorithms for 3SUM}
% \nick{No lower bounds.}

\sout{Towards Polynomial (...), Patrascu: Erikson's problem, Langerman's problem, Pagh's problem, Multiphase problem} % \adam{These are not tight}

\sout{On the Parameterized Complexity of Approximating Dominating Set}

\sout{James King. 2004. A survey of 3SUM-hard problems. 2019?}
% \nick{Mentions only geometric problems, everything is deterministic}

\sout{Unifying and strengthening hardness for dynamic problems via the online matrix-vector multiplication conjecture}

\sout{S. Dahlgaard, “On the hardness of partially dynamic graph problems and connections to diameter”} %\adam{Deterministic reductions from Triangle Connection to 4/3-apx diameter in static and partially dynamic settings}

\sout{Ayelet Butman, Peter Clifford, Raphaël Clifford, Markus Jalsenius, Noa Lewenstein, Benny Porat, Ely Porat, and Benjamin Sach. 2013. Pattern matching under polynomial transformation} % \adam{Almost like geometric reductions, pure algebra}

\sout{JACM A. Grønlund and S. Pettie, Threesomes, degenerates, and love triangles}

\sout{How Fast Can We Play Tetris Greedily With Rectangular Pieces?}

\sout{Smallest k-Enclosing Rectangle Revisited}

\sout{Equivalences between triangle and range query problems}

\sout{Dynamic Parameterized Problems and Algorithms} % \adam{Not tight}

\sout{Fast and Simple Connectivity in Graph Timelines}

\sout{Impossibility Results for Grammar-Compressed Linear Algebra}

\sout{Conditional Lower Bounds for Dynamic Geometric Measure Problems} % \adam{Nothing tight from 3SUM}

\sout{Removing the Haystack to Find the Needle(s): Minesweeper, an Adaptive Join Algorithm}

\sout{Hardness of approximation in P via short cycle removal: cycle detection, distance oracles, and beyond}

\sout{Nearly Optimal Separation Between Partially and Fully Retroactive Data Structures}

\sout{Hardness for triangle problems under even more believable hypotheses: reductions from real APSP, real 3SUM, and OV}

\sout{Translating Hausdorff is Hard: Fine-Grained Lower Bounds for Hausdorff Distance Under Translation}

\sout{Dynamic Set Intersection} % \adam{Not really tight, and not too interesting}

\sout{Fine-grained reductions from approximate counting to decision}

\sout{Joins via Geometric Resolutions: Worst-case and Beyond}

\sout{Fredman's Trick Meets Dominance Product: Fine-Grained Complexity of Unweighted APSP, 3SUM Counting, and More}



\paragraph{Papers on 3XOR.}

Charles Bouillaguet and Claire Delaplace. Faster algorithms for the sparse random 3xor problem

Charles Bouillaguet, Claire Delaplace, and Pierre-Alain Fouque. Revisiting and improving algorithms for the 3xor problem

Martin Dietzfelbinger, Philipp Schlag, and Stefan Walzer. A subquadratic algorithm for 3XOR.

Zahra Jafargholi and Emanuele Viola. 3xor, 3sum, triangles

\paragraph{Other papers.}

Towards Hardness of Approximation for Polynomial Time Problems -- They mention possible deterministic 3SUM Gap Conjecture

Kopelowitz et al. wrote:  "...it would be surprising if our construction can be efficiently derandomized..."

Chan and He wrote: "We leave open the question of whether the dependencies on $U$ could be eliminated in our deterministic reductions  (this  is  related  to  the  question  of  whether 3SUM for arbitrary integers could be reduced deterministically to 3SUM for integers bounded by $n^{O(1)}$), and whether a similar reduction from 3SUM to Convolution-3SUM is possible for real numbers."

Chan, Vassilevska Williams, and Xu~\cite{ChanWX22} give reductions to some triangle problems from 3SUM on real numbers, which is a harder problem than 3SUM on integers. This is another direction in which one can go to strengthen 3SUM-based conditional lower bounds. Their reductions are however not tight. They also use randomization, albeit in a completely different manner, hence our techniques do not seem to apply.

\paragraph{Notes}

Multiphase Problem has a tight reduction from OMv and a non-tight reduction from 3SUM~\cite{Patrascu10}. TODO: Is it randomized?

Dallant and Iacono \cite{DallantI22} give a reduction from Multiphase Problem to a Tetris-inspired data structure that maintains a set of rectangles, and ``supports queries which return where to [greedily] drop the rectangle, and updates which insert a rectangle dropped at a certain position and return the height of the highest point in the updated set of rectangles.''

